Chain of Thoughtlessness? An Analysis of CoT in Planning

Large language model (LLM) performance on reasoning problems typically does not generalize out of distribution. Previous work has claimed that this can be mitigated with chain of thought prompting-a method of demonstrating solution procedures-with the intuition that it is possible to in-context teach an LLM an algorithm for solving the problem. This paper presents a case study of chain of thought on problems from Blocksworld, a classical planning domain, and examines the performance of two state-of-the-art LLMs across two axes: generality of examples given in prompt, and complexity of problems queried with each prompt. While our problems are very simple, we only find meaningful performance improvements from chain of thought prompts when those prompts are exceedingly specific to their problem class, and that those improvements quickly deteriorate as the size n of the query-specified stack grows past the size of stacks shown in the examples. We also create scalable variants of three domains commonly studied in previous CoT papers and demonstrate the existence of similar failure modes. Our results hint that, contrary to previous claims in the literature, CoT's performance improvements do not stem from the model learning general algorithmic procedures via demonstrations but depend on carefully engineering highly problem specific prompts. This spotlights drawbacks of chain of thought, especially the sharp tradeoff between possible performance gains and the amount of human labor necessary to generate examples with correct reasoning traces.

==> prompts/arithm_cot.tex <==
[Instructions]
After each thought, provide an intermediate answer in the form of a single number, labeled by the [Intermediate Answer n] tag, where n is replaced with the number of the intermediate answer. Do not put anything other than the intermediate answer number between the intermediate answer tag and the next thought tag (e.g. [Thought n+1]). When you are done thinking and have outputted all the requisite intermediate answers, put the [Answer] tag. After the [Answer] tag, you may only respond with a single number representing the final value of the calculation. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 3 examples are provided. Please follow the formatting used in them.

Example 0:

[Question]
Simplify the following expression into a single number: 2 + (4)


[Thoughts]
We simplify one set of parentheses at a time, starting from the inside.
[Thought 1]
The current form of the expression is 2 + (4).
The innermost expression is 2 + (4), which simplifies to 6.
The expression cannot be simplified further, so this will also be the final answer.
[Intermediate Answer 1]
6


[Answer]
6

Example 1:

[Question]
Simplify the following expression into a single number: 6 / (7 - (5))


[Thoughts]
We simplify one set of parentheses at a time, starting from the inside.
[Thought 1]
The current form of the expression is 6 / (7 - (5)).
The innermost expression is 7 - (5), which simplifies to 2.
[Intermediate Answer 1]
2
[Thought 2]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 6 / (2).
The innermost expression is 6 / (2), which simplifies to 3.
The expression cannot be simplified further, so this will also be the final answer.
[Intermediate Answer 2]
3


[Answer]
3

Example 2:

[Question]
Simplify the following expression into a single number: 2 / (4 - (9 - (6)))


[Thoughts]
We simplify one set of parentheses at a time, starting from the inside.
[Thought 1]
The current form of the expression is 2 / (4 - (9 - (6))).
The innermost expression is 9 - (6), which simplifies to 3.
[Intermediate Answer 1]
3
[Thought 2]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 2 / (4 - (3)).
The innermost expression is 4 - (3), which simplifies to 1.
[Intermediate Answer 2]
1
[Thought 3]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 2 / (1).
The innermost expression is 2 / (1), which simplifies to 2.
The expression cannot be simplified further, so this will also be the final answer.
[Intermediate Answer 3]
2


[Answer]
2


Problem to solve:

[Question]
Simplify the following expression into a single number: 1 * (1 * (1 * (1 + (8 / (1)))))



[Thoughts]
==================GPT-4-Turbo Response====================
We simplify one set of parentheses at a time, starting from the inside.
[Thought 1]
The current form of the expression is 1 * (1 * (1 * (1 + (8 / (1))))).
The innermost expression is 8 / (1), which simplifies to 8.
[Intermediate Answer 1]
8
[Thought 2]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 1 * (1 * (1 * (1 + (8)))).
The innermost expression is 1 + (8), which simplifies to 9.
[Intermediate Answer 2]
9
[Thought 3]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 1 * (1 * (1 * (9))).
The innermost expression is 1 * (9), which simplifies to 9.
[Intermediate Answer 3]
9
[Thought 4]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 1 * (1 * (9)).
The innermost expression is 1 * (9), which simplifies to 9.
[Intermediate Answer 4]
9
[Thought 5]
We plug in the previous intermediate answer into the previous expression to simplify it by one step. This gives the expression 1 * (9).
The innermost expression is 1 * (9), which simplifies to 9.
The expression cannot be simplified further, so this will also be the final answer.
[Intermediate Answer 5]
9

[Answer]
9

==> prompts/arithm_direct.tex <==
[Instructions]
After the [Answer] tag, you may only respond with a single number representing the final value of the calculation. Do not include anything else after that tag. The [Answer] tag must precede the final answer.
Problem to solve:

[Question]
Simplify the following expression into a single number: 1 * (7 / (5 / (1 + (9 - (5)))))


[Answer]

==================GPT-4-Turbo Response====================
[Answer]
7


==> prompts/arithm_told.tex <==
[Instructions]
After the [Answer] tag, you may only respond with a single number representing the final value of the calculation. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 3 examples are provided. Please follow the formatting used in them.

Example 0:

[Question]
Simplify the following expression into a single number: 2 + (4)
Remember: the final answer and all intermediate answers will be single digit numbers.




[Answer]
6

Example 1:

[Question]
Simplify the following expression into a single number: 6 / (7 - (5))
Remember: the final answer and all intermediate answers will be single digit numbers.




[Answer]
3

Example 2:

[Question]
Simplify the following expression into a single number: 2 / (4 - (9 - (6)))
Remember: the final answer and all intermediate answers will be single digit numbers.




[Answer]
2


Problem to solve:

[Question]
Simplify the following expression into a single number: 1 * (7 / (5 / (1 + (9 - (5)))))
Remember: the final answer and all intermediate answers will be single digit numbers.


[Answer]

==================GPT-4-Turbo Response====================
7

==> prompts/cf_direct.tex <==
[Instructions]
Respond only with 'yes' or 'no'. Do not include anything else in your response.
Problem to solve:

[QUESTION]
A coin is heads up. Craig flips the coin. Is the coin still heads up?


[Answer]
==================GPT-4-Turbo Response====================
no

==> prompts/cf_wei.tex <==
[Instructions]
After the [Answer] tag, you may respond only with 'yes' or 'no'. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 3 examples are provided. Please follow the formatting used in them.

Example 0:

[QUESTION]
A coin is heads up. Craig flips the coin. Is the coin still heads up?


[Thoughts]
The coin was flipped by Craig. So the coin was flipped 1 times. The coin started heads up, so after an odd number of flips, it will be tails up. So the answer is no.

[Answer]
yes

Example 1:

[QUESTION]
A coin is heads up. Major flips the coin. Maria does not flip the coin. Is the coin still heads up?


[Thoughts]
The coin was flipped by Major. So the coin was flipped 1 times. The coin started heads up, so after an odd number of flips, it will be tails up. So the answer is no.

[Answer]
yes

Example 2:

[QUESTION]
A coin is heads up. Albert does not flip the coin. Wolf flips the coin. Page flips the coin. Is the coin still heads up?


[Thoughts]
The coin was flipped by Wolf and Page. So the coin was flipped 2 times. The coin started heads up, so after an even number of flips, it will still be heads up. So the answer is yes.

[Answer]
no


Problem to solve:

[QUESTION]
A coin is heads up. Craig flips the coin. Is the coin still heads up?



[Thoughts]
==================GPT-4-Turbo Response====================
The coin was flipped by Craig. So the coin was flipped 1 time. The coin started heads up, so after an odd number of flips, it will be tails up. So the answer is no.

[Answer]
no


==> prompts/domain_independent.tex <==
The plan correctness is defined in terms of states resulting from executing the actions in the plan. An action is executable in a state when all its preconditions hold in that state. The state resulting from the action execution consists of everything in the previous state with the addition and deletion of add and delete effects of the action. Plan correctness is defined as follows: if the first action in the plan is applicable in the initial state, i.e., its preconditions are all present there; and the second action is applicable in the state resulting from applying the first action to the initial state, this process continues until the state resulting from the application of the last action in the last but one state gives rise to the final state where all the goals are satisfied.

Here is an example problem:

[STATEMENT]
As initial conditions I have that, Block A is clear, Block B is clear, Block C is clear, the hand is empty, Block B is on top of Block D, Block A is on the table, Block D is on the table and Block C is on the table.
My goal is to have that Block D is on top of Block B.

My plan is as follows:

[PLAN]
1. Current State: Block A is clear, Block B is clear, Block C is clear, the hand is empty, Block B is on top of Block D, Block A is on the table, Block C is on the table and Block D is on the table
   Action: unstack Block B from on top of Block D
   Reason: The above action is applicable in the current state because its preconditions; Block B is clear, the hand is empty and Block B is on top of Block D, are satisfied in the current state.
   Resulting State: Block A is clear, Block C is clear, Block D is clear, the hand is currently holding Block B, Block A is on the table, Block C is on the table and Block D is on the table

2. Current State: Block A is clear, Block C is clear, Block D is clear, the hand is currently holding Block B, Block A is on the table, Block C is on the table and Block D is on the table
   Action: put down Block B
   Reason: The above action is applicable in the current state because its preconditions; the hand is currently holding Block B, are satisfied in the current state.
   Resulting State: Block A is clear, Block B is clear, Block C is clear, Block D is clear, the hand is empty, Block A is on the table, Block B is on the table, Block C is on the table and Block D is on the table

3. Current State: Block A is clear, Block B is clear, Block C is clear, Block D is clear, the hand is empty, Block A is on the table, Block B is on the table, Block C is on the table and Block D is on the table
   Action: pick up Block D
   Reason: The above action is applicable in the current state because its preconditions; Block D is clear, the hand is empty and Block D is on the table, are satisfied in the current state.
   Resulting State: Block A is clear, Block B is clear, Block C is clear, the hand is currently holding Block D, Block A is on the table, Block B is on the table and Block C is on the table

4. Current State: Block A is clear, Block B is clear, Block C is clear, the hand is currently holding Block D, Block A is on the table, Block B is on the table and Block C is on the table
   Action: stack Block D on top of Block B
   Reason: The above action is applicable in the current state because its preconditions; Block B is clear and the hand is currently holding Block D, are satisfied in the current state.
   Resulting State: Block A is clear, Block C is clear, Block D is clear, the hand is empty, Block D is on top of Block B, Block A is on the table, Block B is on the table and Block C is on the table

Final State: Block A is clear, Block C is clear, Block D is clear, the hand is empty, Block D is on top of Block B, Block A is on the table, Block B is on the table and Block C is on the table
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]

Here is another example:

[STATEMENT]
As initial conditions I have that, Block B is clear, Block B is on top of Block C, Block C is on top of Block A, the hand is empty, Block A is on the table, and Block D is on the table.
My goal is to have that Block C is on top of Block B and Block D is on top of Block C.

My plan is as follows:

[PLAN]
1. Current State: the Block B is clear, the Block D is clear, the hand is empty, the Block B is on top of the Block C, the Block C is on top of the Block A, the Block A is on the table and the Block D is on the table
   Action: unstack the Block B from on top of the Block C
   Reason: The above action is applicable in the current state because its preconditions; the Block B is clear, the hand is empty and the Block B is on top of the Block C, are satisfied in the current state.
   Resulting State: the Block C is clear, the Block D is clear, the hand is currently holding Block B, the Block C is on top of the Block A, the Block A is on the table and the Block D is on the table

2. Current State: the Block C is clear, the Block D is clear, the hand is currently holding Block B, the Block C is on top of the Block A, the Block A is on the table and the Block D is on the table
   Action: put down the Block B
   Reason: The above action is applicable in the current state because its preconditions; the hand is currently holding Block B, are satisfied in the current state.
   Resulting State: the Block B is clear, the Block C is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block A, the Block A is on the table, the Block B is on the table and the Block D is on the table

3. Current State: the Block B is clear, the Block C is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block A, the Block A is on the table, the Block B is on the table and the Block D is on the table
   Action: unstack the Block C from on top of the Block A
   Reason: The above action is applicable in the current state because its preconditions; the Block C is clear, the hand is empty and the Block C is on top of the Block A, are satisfied in the current state.
   Resulting State: the Block A is clear, the Block B is clear, the Block D is clear, the hand is currently holding Block C, the Block A is on the table, the Block B is on the table and the Block D is on the table

4. Current State: the Block A is clear, the Block B is clear, the Block D is clear, the hand is currently holding Block C, the Block A is on the table, the Block B is on the table and the Block D is on the table
   Action: stack the Block C on top of the Block B
   Reason: The above action is applicable in the current state because its preconditions; the Block B is clear and the hand is currently holding Block C, are satisfied in the current state.
   Resulting State: the Block A is clear, the Block C is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block B, the Block A is on the table, the Block B is on the table and the Block D is on the table

5. Current State: the Block A is clear, the Block C is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block B, the Block A is on the table, the Block B is on the table and the Block D is on the table
   Action: pick up the Block D
   Reason: The above action is applicable in the current state because its preconditions; the Block D is clear, the hand is empty and the Block D is on the table, are satisfied in the current state.
   Resulting State: the Block A is clear, the Block C is clear, the hand is currently holding Block D, the Block C is on top of the Block B, the Block A is on the table and the Block B is on the table

6. Current State: the Block A is clear, the Block C is clear, the hand is currently holding Block D, the Block C is on top of the Block B, the Block A is on the table and the Block B is on the table
   Action: stack the Block D on top of the Block C
   Reason: The above action is applicable in the current state because its preconditions; the Block C is clear and the hand is currently holding Block D, are satisfied in the current state.
   Resulting State: the Block A is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block B, the Block D is on top of the Block C, the Block A is on the table and the Block B is on the table

Final State: the Block A is clear, the Block D is clear, the hand is empty, the Block C is on top of the Block B, the Block D is on top of the Block C, the Block A is on the table and the Block B is on the table
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]
Here is the problem to solve:

[STATEMENT]
As initial conditions I have that: Block B is clear, Block C is clear, the hand is empty, Block B is on top of Block A, Block A is on the table and Block C is on the table.
My goal is for the following to be true: Block A is on top of Block B and Block C is on top of Block A.

My plan is as follows:

==================GPT-4 Response====================

[PLAN]
1. Current State: Block B is clear, Block C is clear, the hand is empty, Block B is on top of Block A, Block A is on the table and Block C is on the table
   Action: unstack Block B from on top of Block A
   Reason: The above action is applicable in the current state because its preconditions; Block B is clear, the hand is empty and Block B is on top of Block A, are satisfied in the current state.
   Resulting State: Block A is clear, Block C is clear, the hand is currently holding Block B, Block A is on the table and Block C is on the table

2. Current State: Block A is clear, Block C is clear, the hand is currently holding Block B, Block A is on the table and Block C is on the table
   Action: put down Block B
   Reason: The above action is applicable in the current state because its preconditions; the hand is currently holding Block B, are satisfied in the current state.
   Resulting State: Block A is clear, Block B is clear, Block C is clear, the hand is empty, Block A is on the table, Block B is on the table and Block C is on the table

3. Current State: Block A is clear, Block B is clear, Block C is clear, the hand is empty, Block A is on the table, Block B is on the table and Block C is on the table
   Action: pick up Block A
   Reason: The above action is applicable in the current state because its preconditions; Block A is clear, the hand is empty and Block A is on the table, are satisfied in the current state.
   Resulting State: Block B is clear, Block C is clear, the hand is currently holding Block A, Block B is on the table and Block C is on the table

4. Current State: Block B is clear, Block C is clear, the hand is currently holding Block A, Block B is on the table and Block C is on the table
   Action: stack Block A on top of Block B
   Reason: The above action is applicable in the current state because its preconditions; Block B is clear and the hand is currently holding Block A, are satisfied in the current state.
   Resulting State: Block A is clear, Block C is clear, the hand is empty, Block A is on top of Block B, Block B is on the table and Block C is on the table

5. Current State: Block A is clear, Block C is clear, the hand is empty, Block A is on top of Block B, Block B is on the table and Block C is on the table
   Action: pick up Block C
   Reason: The above action is applicable in the current state because its preconditions; Block C is clear, the hand is empty and Block C is on the table, are satisfied in the current state.
   Resulting State: Block A is clear, the hand is currently holding Block C, Block A is on top of Block B and Block B is on the table

6. Current State: Block A is clear, the hand is currently holding Block C, Block A is on top of Block B and Block B is on the table
   Action: stack Block C on top of Block A
   Reason: The above action is applicable in the current state because its preconditions; Block A is clear and the hand is currently holding Block C, are satisfied in the current state.
   Resulting State: Block C is clear, the hand is empty, Block A is on top of Block B, Block C is on top of Block A and Block B is on the table

Final State: Block C is clear, the hand is empty, Block A is on top of Block B, Block C is on top of Block A and Block B is on the table
The goal conditions are satisfied in the final state. Hence, the above plan is valid.
[PLAN END]

==================VALID PLAN====================

==> prompts/domain_prompt.tex <==
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.
Once you stack a block on top of a second block, the second block is no longer clear.

==> prompts/domain_specific.tex <==
Here is an example problem:

[STATEMENT]
As initial conditions I have that, Block B is clear, Block C is clear, the hand is empty, Block C is on top of Block A, Block A is on the table, Block B is on the table.
My goal is to have that Block A is on top of Block C and Block B is on top of Block A

My plan is as follows:

[THOUGHTS]
1. I take apart all the towers, and put all the blocks on the table.
I will check every block. Any that are already on the table can be left there. Any that are on top of another block must be put on the table, but I can only unstack them if they are clear, so I will check that before trying to unstack any of them. If a block needs to be moved but isn't clear, I'll come back to it later once it is. 

Block A is already on the table but is not clear.
Block B is already on the table.
Block C is on top of Block A. I can only unstack a block that is clear. C is clear according to the initial condition, so I can proceed. I unstack it. Then, I put it down on the table. This clears Block A.

All the blocks are now clear and on the table.

2. I look at the goal and stack each tower I need, starting from the bottom. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block A needs to be on top of Block C, so it can't be the base of a tower.
Block B needs to be on top of Block A, so it can't be the base of a tower.
Block C needs Block A on top of it. I double check the goal: this is the only condition that must hold for block C. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.

In summary, only Block C can be used as a base of a tower.

I build the tower that has Block C as a base. I don't need to move Block C, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block C is Block A. I pick up Block A. I stack it on top of Block C.
The block that goes on top of Block A is Block B. I pick up Block B. I stack it on top of Block A. 
No block needs to be on top of Block B. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

3. Now, I write down my plan in the required format:

[PLAN]
unstack Block C from on top of Block A
put down Block C
pick up Block A
stack Block A on top of Block C
pick up Block B
stack Block B on top of Block A
[PLAN END]

Here is another example:

[STATEMENT]
As initial conditions I have that, Block B is clear, the hand is empty, Block A is on top of Block D, Block B is on top of Block C, Block C is on top of Block A and Block D is on the table.
My goal is to have that Block C is on top of Block D, Block A is on top of Block C and Block B is on top of Block A.

My plan is as follows:

[THOUGHTS]
1. I take apart all the towers, and put all the blocks on the table.
I will check every block. Any that are already on the table can be left there. Any that are on top of another block must be put on the table, but I can only unstack them if they are clear, so I will check that before trying to unstack any of them. If a block needs to be moved but isn't clear, I'll come back to it later once it is. 

Block A is on top of Block D. I can only unstack a block that is clear. The initial condition states that Block C is on top of Block A. Therefore, I can't unstack Block A until I move Block C. I don't touch it yet, and look at Block C.
Block C is on top of Block A. I can only unstack a block that is clear. The initial condition states that Block B is on top of Block C. Therefore, I can't unstack Block C until I move Block B. I don't touch it yet, and look at Block B.
Block B is on top of Block C. I can only unstack a block that is clear. The initial condition states that Block B is clear. I unstack it. Then, I put it down on the table. This clears Block C.
Block C is on top of Block A. I can only unstack a block that is clear. Block C is cleared previously. I unstack it. Then, I put it down on the table. This clears Block A.
Block A is on top of Block D. I can only unstack a block that is clear. Block A is cleared previously. I unstack it. Then, I put it down on the table. This clears Block D.

All the blocks are now clear and on the table.

2. I look at the goal and stack each tower I need, starting from the bottom. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block C needs to be on top of Block D, so it can't be the base of a tower.
Block A needs to be on top of Block C, so it can't be the base of a tower.
Block B needs to be on top of Block A, so it can't be the base of a tower.
Block D needs Block C on top of it. I double check the goal: this is the only condition that must hold for block D. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.

In summary, only Block D can be used as the base of a tower.

I build the tower that has Block D as a base. I don't need to move Block D, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block D is Block C. I pick up Block C. I stack it on top of Block D.
The block that goes on top of Block C is Block A. I pick up Block A. I stack it on top of Block C.
The block that goes on top of Block A is Block B. I pick up Block B. I stack it on top of Block A.
No block needs to be on top of Block B. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

3. Now, I write down my plan in the required format:

[PLAN]
unstack Block B from on top of Block C
put down Block B
unstack Block C from on top of Block A
put down Block C
unstack Block A from on top of Block D
put down Block A
pick up Block C
stack Block C on top of Block D
pick up Block A
stack Block A on top of Block C
pick up Block B
stack Block B on top of Block A
[PLAN END]
Here is the problem to solve:

[STATEMENT]
As initial conditions I have that: Block B is clear, Block C is clear, the hand is empty, Block B is on top of Block A, Block A is on the table and Block C is on the table.
My goal is for the following to be true: Block A is on top of Block B and Block C is on top of Block A.

My plan is as follows:

==================GPT-4 Response====================
[THOUGHTS]
1. I take apart all the towers, and put all the blocks on the table.
I will check every block. Any that are already on the table can be left there. Any that are on top of another block must be put on the table, but I can only unstack them if they are clear, so I will check that before trying to unstack any of them. If a block needs to be moved but isn't clear, I'll come back to it later once it is. 

Block A is on the table but is not clear.
Block B is on top of Block A. I can only unstack a block that is clear. B is clear according to the initial condition, so I can proceed. I unstack it. Then, I put it down on the table. This clears Block A.
Block C is already on the table.

All the blocks are now clear and on the table.

2. I look at the goal and stack each tower I need, starting from the bottom. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block A needs to be on top of Block B, so it can't be the base of a tower.
Block B needs Block A on top of it. I double check the goal: this is the only condition that must hold for block B. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.
Block C needs to be on top of Block A, so it can't be the base of a tower.

In summary, only Block B can be used as the base of a tower.

I build the tower that has Block B as a base. I don't need to move Block B, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block B is Block A. I pick up Block A. I stack it on top of Block B.
The block that goes on top of Block A is Block C. I pick up Block C. I stack it on top of Block A. 
No block needs to be on top of Block C. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

3. Now, I write down my plan in the required format:

[PLAN]
unstack Block B from on top of Block A
put down Block B
pick up Block A
stack Block A on top of Block B
pick up Block C
stack Block C on top of Block A
[PLAN END]
==================VALID PLAN====================

==> prompts/goal_class_specific.tex <==
STATEMENT]
As initial conditions I have that, Block A is clear, Block B is clear, Block A is on the table, Block B is on the table and the hand is empty.
My goal is to have that Block B is on top of Block A.

My plan is as follows:

[THOUGHTS]
1. I look at the goal and stack each tower I need, starting from the bottom.
My goal only mentions blocks B and A. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block A needs to have Block B on top of it. I double check the goal: this is the only condition that must hold for block A. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.
Block B needs to be on top of Block A, so it can't be the base of a tower.

In summary, only Block A can be used as a base of a tower.

I build the tower that has Block A as a base. I don't need to move Block A, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block A is Block B. I pick up Block B. I stack it on top of Block A.
This satisfies the part of the goal that says that Block B is on top of Block A.
No block needs to be on top of Block B. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

2. Now, I write down my plan in the required format:

[PLAN]
pick up Block B
stack Block B on top of Block A
[PLAN END]

Here is another example:

[STATEMENT]
As initial conditions I have that, Block A is clear, Block B is clear, Block C is clear, Block A is on the table, Block B is on the table, Block C is on the table and the hand is empty.
My goal is to have that Block A is on top of Block C and Block B is on top of Block A.

My plan is as follows:

[THOUGHTS]
1. I look at the goal and stack each tower I need, starting from the bottom.
My goal only mentions blocks A, B, and C. I am free to ignore all other blocks. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block C needs Block A on top of it. I double check the goal: this is the only condition that must hold for block C. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.
Block A needs Block B on top of it. I double check the goal: this isn't the only condition that must hold for Block A, because Block A needs to be on top of Block C. Therefore Block A can't be the base of a tower.
Block B needs to be on top of Block A, so it can't be the base of a tower.

In summary, only Block C can be used as the base of a tower.

I build the tower that has Block C as a base. I don't need to move Block C, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block C is Block A. I pick up Block A. I stack it on top of Block C.
This satisfies the part of the goal that says that Block A is on top of Block C.
The block that goes on top of Block A is Block B. I pick up Block B. I stack it on top of Block A.
This satisfies the part of the goal that says that Block B is on top of Block A.
No block needs to be on top of Block B. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

2. Now, I write down my plan in the required format:

[PLAN]
pick up Block A
stack Block A on top of Block C
pick up Block B
stack Block B on top of Block A
[PLAN END]
Here is the problem to solve:

[STATEMENT]
As initial conditions I have that: Block A is clear, Block B is clear, Block C is clear, the hand is empty, Block A is on the table, Block B is on the table and Block C is on the table.
My goal is for the following to be true: Block A is on top of Block B and Block C is on top of Block A.

My plan is as follows:

==================GPT-4 Response====================
[THOUGHTS]
1. I look at the goal and stack each tower I need, starting from the bottom.
My goal only mentions blocks A, B, and C. I am free to ignore all other blocks. I check each of the mentioned blocks in order to determine which of them are the bases of towers.

Block B needs Block A on top of it. I double check the goal: this is the only condition that must hold for block B. It does not need to be on top of any other block. Therefore, I can use it as the base of a tower.
Block A needs Block C on top of it. I double check the goal: this isn't the only condition that must hold for Block A, because Block A needs to be on top of Block B. Therefore Block A can't be the base of a tower.
Block C needs to be on top of Block A, so it can't be the base of a tower.

In summary, only Block B can be used as the base of a tower.

I build the tower that has Block B as a base. I don't need to move Block B, and I leave it be, as I know it is already placed correctly.
The block that goes on top of Block B is Block A. I pick up Block A. I stack it on top of Block B.
This satisfies the part of the goal that says that Block A is on top of Block B.
The block that goes on top of Block A is Block C. I pick up Block C. I stack it on top of Block A.
This satisfies the part of the goal that says that Block C is on top of Block A.
No block needs to be on top of Block C. Therefore this tower is complete.

There are no other blocks which can be used as a base of a tower, and all the blocks mentioned in the goal have been placed, so I am done constructing.

2. Now, I write down my plan in the required format:

[PLAN]
pick up Block A
stack Block A on top of Block B
pick up Block C
stack Block C on top of Block A
[PLAN END]
==================VALID PLAN====================

==> prompts/goal_specific.tex <==
Here is an example problem:

[STATEMENT]
As initial conditions I have that, Block A is clear, Block B is clear, Block A is on the table, Block B is on the table and the hand is empty.
My goal is to have that Block A is on top of Block B.

My plan is as follows:

[THOUGHTS]
1. I look at the goal and stack the tower I need, starting from the bottom.
Block B is on the table and Block B is clear.
Block A is on the table and Block A is clear, so I pick it up.
Then, I stack Block A on top of Block B. The goal conditions are satisfied.


2. Now, I write down my plan in the required format:

[PLAN]
pick up Block A
stack Block A on top of Block B
[PLAN END]

Here is another example:

[STATEMENT]
As initial conditions I have that, Block A is clear, Block B is clear, Block C is clear, Block A is on the table, Block B is on the table, Block C is on the table and the hand is empty.
My goal is to have that Block A is on top of Block B and Block B is on top of Block C.

My plan is as follows:

[THOUGHTS]
1. I look at the goal and stack the tower I need, starting from the bottom.
Block C is on the table and Block C is clear.
Block B is on the table and Block B is clear, so I pick it up.
Then, I stack Block B on top of Block C. The first goal condition is satisfied.
Block A is on the table and Block A is clear, so I pick it up.
Then, I stack Block A on top of Block B. The second goal condition is satisfied.
So all goal conditions are satisfied.


2. Now, I write down my plan in the required format:

[PLAN]
pick up Block B
stack Block B on top of Block C
pick up Block A
stack Block A on top of Block B
[PLAN END]
Here is the problem to solve:

[STATEMENT]
As initial conditions I have that: Block A is clear, Block B is clear, Block C is clear, Block D is clear, the hand is empty, Block A is on the table, Block B is on the table, Block C is on the table and Block D is on the table.
My goal is for the following to be true: Block A is on top of Block B, Block B is on top of Block C and Block C is on top of Block D.

My plan is as follows:

==================GPT-4 Response====================
[THOUGHTS]
1. I look at the goal and stack the tower I need, starting from the bottom.
Block D is on the table and Block D is clear.
Block C is on the table and Block C is clear, so I pick it up.
Then, I stack Block C on top of Block D. The first goal condition is satisfied.
Block B is on the table and Block B is clear, so I pick it up.
Then, I stack Block B on top of Block C. The second goal condition is satisfied.
Block A is on the table and Block A is clear, so I pick it up.
Then, I stack Block A on top of Block B. The third goal condition is satisfied.
So all goal conditions are satisfied.

2. Now, I write down my plan in the required format:

[PLAN]
pick up Block C
stack Block C on top of Block D
pick up Block B
stack Block B on top of Block C
pick up Block A
stack Block A on top of Block B
[PLAN END]
==================VALID PLAN====================

==> prompts/llc_direct.tex <==
[Instructions]
After the [Answer] tag, you may only respond with a lowercase string of concatenated characters. Do not include anything else after that tag. The [Answer] tag must precede the final answer.
Problem to solve:

[Question]
Take the last letters of each word in "Analy Daniel" and concatenate them.

 

[Thoughts]
==================GPT-4-Turbo Response====================
[Answer] yy

==> prompts/llc_foom.tex <==
[Instructions]
After the [Answer] tag, you may only respond with a lowercase string of concatenated characters. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 2 examples are provided. Please follow the formatting used in them.

Example 0:

[Question]
Take the following words and produce a new string using them: "Anthony". The first letter of your string should be the first letter of the first word, the second letter of your string should be the second letter of the second word, and so forth. If you need the nth letter of the nth word, but that word is less than n letters long, then insert a 0 character instead.


[Thoughts]
The 1st letter of "Anthony" is A. Concatenating them is "a". The answer is a.

[Answer]
a

Example 1:

[Question]
Take the following words and produce a new string using them: "Beautiful Ash". The first letter of your string should be the first letter of the first word, the second letter of your string should be the second letter of the second word, and so forth. If you need the nth letter of the nth word, but that word is less than n letters long, then insert a 0 character instead.


[Thoughts]
The 1st letter of "Beautiful" is B. The 2nd letter of "Ash" is s. Concatenating them is "bs". The answer is bs.

[Answer]
bs


Problem to solve:

[Question]
Take the following words and produce a new string using them: "Analy Daniel". The first letter of your string should be the first letter of the first word, the second letter of your string should be the second letter of the second word, and so forth. If you need the nth letter of the nth word, but that word is less than n letters long, then insert a 0 character instead.



[Thoughts]

==================GPT-4-Turbo Response====================
The 1st letter of "Analy" is A. The 2nd letter of "Daniel" is a. The 3rd letter of "Analy" is a. The 4th letter of "Daniel" is i. The 5th letter of "Analy" is y. The 6th letter of "Daniel" is e. Concatenating them is "Aaaiye". The answer is aaaiye.

[Answer]
aaaiye


==> prompts/llc_vowel.tex <==
[Instructions]
For the purposes of these problems, a vowel is any one of the letters "a","e","i","o", or "u", but NOT "y". After the [Answer] tag, you may only respond with a lowercase string of concatenated characters. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 3 examples are provided. Please follow the formatting used in them.

Example 0:

[Question]
Take the last vowel of each word in "Anthony" and concatenate them.




[Answer]
o

Example 1:

[Question]
Take the last vowel of each word in "Beautiful Ash" and concatenate them.




[Answer]
ua

Example 2:

[Question]
Take the last vowel of each word in "Matthew River Craig" and concatenate them.




[Answer]
eei


Problem to solve:

[Question]
Take the last vowel of each word in "Analy Daniel" and concatenate them.


[Answer]

==================GPT-4-Turbo Response====================
ya

==> prompts/llc_wei.tex <==
[Instructions]
After the [Answer] tag, you may only respond with a lowercase string of concatenated characters. Do not include anything else after that tag. The [Answer] tag must precede the final answer.

The following 3 examples are provided. Please follow the formatting used in them.

Example 0:

[Question]
Take the last letters of each word in "Anthony" and concatenate them.


[Thoughts]
The last letter of "Anthony" is y. Concatenating them is "y". The answer is y.

[Answer]
y

Example 1:

[Question]
Take the last letters of each word in "Beautiful Ash" and concatenate them.


[Thoughts]
The last letter of "Beautiful" is l. The last letter of "Ash" is h. Concatenating them is "lh". The answer is lh.

[Answer]
lh

Example 2:

[Question]
Take the last letters of each word in "Matthew River Craig" and concatenate them.


[Thoughts]
The last letter of "Matthew" is w. The last letter of "River" is r. The last letter of "Craig" is g. Concatenating them is "wrg". The answer is wrg.

[Answer]
wrg


Problem to solve:

[Question]
Take the last letters of each word in "Analy Daniel" and concatenate them.



[Thoughts]
==================GPT-4-Turbo Response====================
The last letter of "Analy" is y. The last letter of "Daniel" is l. Concatenating them is "yl". The answer is yl.

[Answer]
yl

==> prompts/mapping.tex <==
I am playing with a set of objects. Here are the actions I can do      
    Attack object
    Feast object from another object
    Succumb object
    Overcome object from another object  
I have the following restrictions on my actions:
      To perform Attack action, the following facts need to be true: Province object, Planet object, Harmony.
      Once Attack action is performed the following facts will be true: Pain object.
      Once Attack action is performed the following facts will be false: Province object, Planet object, Harmony.
      To perform Succumb action, the following facts need to be true: Pain object.
      Once Succumb action is performed the following facts will be true: Province object, Planet object, Harmony.
      Once Succumb action is performed the following facts will be false: Pain object.
      To perform Overcome action, the following needs to be true: Province other object, Pain object.
      Once Overcome action is performed the following will be true: Harmony, Province object, Object Craves other object.
      Once Overcome action is performed the following will be false: Province other object, Pain object.
      To perform Feast action, the following needs to be true: Object Craves other object, Province object, Harmony.
      Once Feast action is performed the following will be true: Pain object, Province other object.
      Once Feast action is performed the following will be false:, Object Craves other object, Province object, Harmony.

You will be given a set of initial conditions and a goal condition. To solve the problem, you will have to tell me which actions to take and in which order in order to achieve the goal.


Please provide your answers using the above terminology. However, you may find it helpful to translate the above description into a common-sense format while working out your solution. Just remember to translate it back later!
Instead of thinking in terms of "objects", think in terms of different alphabet blocks (block A, block B, etc.) which you are stacking (using just one hand) in towers on a table.

Then the "facts" that are true or false at a given time are really facts about the blocks and the hand:
      "Province object a" just means that "block A is clear" or, equivalently, "nothing is on top of block A"
      "Planet object a" is another way of saying "block A is on the table"
      "Harmony" is a codeword for "my hand isn't holding anything"
      "Pain object a" = "the hand is holding block A"
      "object a Craves object b" translates to "block A is on top of block B"

And the "actions" can be seen as stacking and unstacking of blocks (where the restrictions stop us from picking up the bottom block in a tower or holding more than one block in the hand at a time):
      "Attack object a" translates to "pick up block A directly from the table"
      "Feast object a from object b" translates to "pick up block A from directly on top of block B"
      "Succumb object a" translates to "put block A directly on the table"
      "Overcome object a from object b" translates to "put block A directly on top of block B"
      

If you do use this framing, make sure to remember to translate back into the original terms. 

[STATEMENT]
As initial conditions I have that: object b craves object a, object c craves object b, harmony, planet object a and province object c.
My goal is for the following to be true: object a craves object b and object c craves object a.

My plan is as follows:

[PLAN]
feast object c from object b
succumb object c
feast object b from object a
succumb object b
attack object a
overcome object a from object b
attack object c
overcome object c from object a
[PLAN END]

[STATEMENT]
As initial conditions I have that: harmony, planet object a, planet object b, planet object c, province object a, province object b and province object c.
My goal is for the following to be true: object a craves object c and object b craves object a.

My plan is as follows:

[PLAN]
===============GPT-4 Response=================
attack object a
overcome object a from object c
attack object b
overcome object b from object a
[PLAN END]
==================VALID PLAN====================


===============Claude-3-Opus Response=================
Here is a plan to achieve the goal state from the given initial conditions:

attack object a
overcome object a from object c
attack object b 
overcome object b from object a
succumb object b
succumb object a

To explain:
1. Pick up block A from the table. 
2. Put block A on top of block C.
3. Pick up block B from the table.
4. Put block B on top of block A.
5. Put block B down on the table.
6. Put block A down on the table.

This will result in the goal state of block A being on top of block C, and block B being on top of block A.

[PLAN END]
==================INVALID PLAN====================
